Safe Control Synthesis with Uncertain Dynamics and Constraints

This paper considers safe control synthesis for dynamical systems with either probabilistic or worst-case uncertainty in both the dynamics model and the safety constraints. We formulate novel probabilistic and robust (worst-case) control Lyapunov function (CLF) and control barrier function (CBF) constraints that take into account the effect of uncertainty in either case. We show that either the probabilistic or the robust (worst-case) formulation leads to a second-order cone program (SOCP), which enables efficient safe and stable control synthesis. We evaluate our approach in PyBullet simulations of an autonomous robot navigating in unknown environments and compare the performance with a baseline CLF-CBF quadratic programming approach.

==> tex/3_Estimation.tex <==
\section{Environment and System Dynamics Estimation}

In this section, we propose our approach to learn the system dynamics with uncertainty offline and estimate barrier functions for robots operating in some unknown environments online. 

\subsection{Online Bayesian Signed Distance Function Learning}














\subsection{Bayesian System Dynamics Learning}
After addressing the problem of estimating SDFs online, we also need to deal with Problem~\ref{prob: estimate_dynamics}. Recently, the idea of incorporating neural networks with physics laws has becoming more and more popular. 



 

==> tex/3_Moving_Objects.tex <==
\section{Safety with Time-Dependent Control Barrier Functions} 
We use the following Lie-derivative notations for the given time-varying barrier function $h(\boldsymbol{x},t)$: 
\begin{equation}
% \label{eq: lie-derivative}
\begin{aligned}
\mathcal{L}_f h(\boldsymbol{x},t) = \frac{\partial h}{\partial \boldsymbol{x}}(\boldsymbol{x},t)f(\boldsymbol{x}), \quad \mathcal{L}_g h(\boldsymbol{x},t) = \frac{\partial h}{\partial \boldsymbol{x}}(\boldsymbol{x},t)g(\boldsymbol{x})
\end{aligned}
\end{equation}

\begin{align}
    \frac{\partial h(\bfx, \bfy(t))}
    {\partial t} = \frac{\partial h(\bfx, \bfy(t))}{\partial \bfx} 
    (f(\bfx) + g(\bfx)\bfu) + \frac{\partial h(\bfx, \bfy(t))}{\partial \bfy}\dot{\bfy}
\end{align}


consider the following QP problem for safe controller synthesis: 
\begin{equation}
\label{eq:QP_moving}
\begin{aligned}
& \min_{\boldsymbol{u} \in \calU,\delta \in \bbR}\,\, \|L(\boldsymbol{x})^\top(\boldsymbol{u} - \tilde{\boldsymbol{u}}(\boldsymbol{x}))\|^2 + \lambda \delta^2\\
% \boldsymbol{u}^T H \boldsymbol{u} + p_d \delta^2 \\
\mathrm{s.t.} \, \,  &\mathcal{L}_f V(\boldsymbol{x}) + \mathcal{L}_g V(\boldsymbol{x})  \boldsymbol{u} + \alpha_V(V(\boldsymbol{x})) \leq \delta \\
&\mathcal{L}_{f} h(\boldsymbol{x},t) + \mathcal{L}_{g} h(\boldsymbol{x,t})\boldsymbol{u} + \alpha_h(h(\boldsymbol{x},t)) \geq 0,
\end{aligned}
\end{equation}

==> tex/Preliminaries.tex <==

% \subsection{Related work for reference}
% 1. On products of Gaussian random variables %https://arxiv.org/pdf/1711.10516.pdf

% 2. Products of Gaussians %https://papers.nips.cc/paper/2001/file/8232e119d8f59aa83050a741631803a6-Paper.pdf

\section{Preliminaries}
\label{sec:preliminary}
\subsection{Signed Distance Function}
Throughout the paper, we use the concept of signed distance function (SDF) to describe each unsafe region $\{v(\mathcal{O}_i)\}_{i=1}^K$. For each $i$, the SDF function $\varphi_i: \mathcal{Y} \mapsto \mathbb{R}$ is:
\begin{equation}
\varphi_{i}(\boldsymbol{y}) := \begin{cases}
 -d(\boldsymbol{y},\partial v(\calO_i)), & \boldsymbol{y} \in v(\calO_i), \\
 \phantom{-} d(\boldsymbol{y},\partial v(\calO_i)), &  \boldsymbol{y} \notin v(\calO_i),
 \end{cases}
\end{equation} 
where $d$ denotes the Euclidean distance between a point and a set. 

\subsection{Control Lyapunov Function}

A \emph{control Lyapunov function (CLF)} for the system dynamics in \eqref{eq: dynamic} is a continuously differentiable function $V: \mathbb{R}^n \mapsto {\mathbb{R}_{\geq 0}}$ for which there exist a class $\mathcal{K}$ function $\alpha_V$ such that, for all $\boldsymbol{x} \in \mathcal{X}$:
% \NA{Why do we commit to a constant $c_3$ instead of a class $\calK$ function?}
\begin{align*}
    % c_1\|\boldsymbol{x}\|^2 \leq &V(\boldsymbol{x}) \leq c_2\|\boldsymbol{x}\|^2\\
    \inf_{\boldsymbol{u}\in \mathcal{U}}[ \mathcal{L}_f V(\boldsymbol{x}) + \mathcal{L}_g V(\boldsymbol{x})\boldsymbol{u} + \alpha_V( V(\boldsymbol{x}))  ] \leq 0 .
\end{align*}


The function $V$ may be used to encode a variety of control objectives, including path following.

\subsection{Control Barrier Function}

% A useful tool to ensure that the robot state remains in the safe set $\mathcal{S}$ throughout its evolution is the notion of control barrier function (CBF). The definition of the lie-derivative along some matrix $g(\boldsymbol{x})$ is given as follows:


% \begin{align}
%     \calL_g h(\boldsymbol{x}) = [\nabla_{\boldsymbol{x}} h(\boldsymbol{x})]^\top g(\boldsymbol{x}) \in \bbR^{1 \times m}
% \end{align}

\begin{definition}[{\cite{ames2016control}}]
A continuously differentiable function $h: \mathbb{R}^n \mapsto {\mathbb{R}}$, with $h(\boldsymbol{x}) >0$ if $\boldsymbol{x} \in \operatorname{Int}(\mathcal{S})$ and $h(\boldsymbol{x}) =0$ if $\boldsymbol{x} \in \partial \mathcal{S}$, is a \emph{zeroing control barrier function (ZCBF)} on $\mathcal{X} \subset \mathbb{R}^n$ if there exists an extended class $\mathcal{K}$ function $\alpha_h$ such that, for each $\boldsymbol{x} \in \mathcal{X}$, there exists $\boldsymbol{u} \in \mathcal{U}$ with
\begin{equation}\label{eq:cbf}
    \mathcal{L}_f h(\boldsymbol{x}) + \mathcal{L}_g h(\boldsymbol{x})\boldsymbol{u} + \alpha_h (h(\boldsymbol{x})) \geq 0,
\end{equation}
where $\mathcal{L}_f h(\boldsymbol{x})$ is the Lie derivative of $h(\boldsymbol{x})$ along $f(\boldsymbol{x})$.
\end{definition}


Any Lipschitz-continuous controller $\boldsymbol{u}: \mathcal{X} \mapsto \mathcal{U}$ such that $\boldsymbol{u}(\boldsymbol{x})$ satisfies \eqref{eq:cbf} renders the set $\mathcal{S}$ forward invariant for the control-affine system \eqref{eq: dynamic} \cite{cbf, ames2016control}. 

When the barrier function is precisely known, one can combine CLF and CBF constraints to synthesize a safe controller via the following QP:
\begin{equation}
\label{eq:QP_origin}
\begin{aligned}
& \min_{\boldsymbol{u} \in \calU,\delta \in \bbR}\,\, \|L(\boldsymbol{x})^\top(\boldsymbol{u} - \tilde{\boldsymbol{u}}(\boldsymbol{x}))\|^2 + \lambda \delta^2\\
% \boldsymbol{u}^T H \boldsymbol{u} + p_d \delta^2 \\
\mathrm{s.t.} \, \,  &\mathcal{L}_f V(\boldsymbol{x}) + \mathcal{L}_g V(\boldsymbol{x})  \boldsymbol{u} + \alpha_V(V(\boldsymbol{x})) \leq \delta \\
&\mathcal{L}_{f} h(\boldsymbol{x}) + \mathcal{L}_{g} h(\boldsymbol{x})\boldsymbol{u} + \alpha_h(h(\boldsymbol{x})) \geq 0,
\end{aligned}
\end{equation}

where $\tilde{\boldsymbol{u}}(\boldsymbol{x})$ is a baseline controller, $L(\bfx)$ is a matrix penalizing control effort, and $\delta \geq 0$ (with the corresponding penalty $\lambda$) is a slack variable, introduced to relax the CLF constraints in order to ensure the feasibility of the QP. The baseline controller $\tilde{\boldsymbol{u}}(\boldsymbol{x})$ is used to specify additional control requirements such as desirable velocity or orientation but may be set to $\tilde{\boldsymbol{u}}(\boldsymbol{x}) \equiv 0$ if minimum control effort is the main objective. The QP formulation in \eqref{eq:QP_origin} modifies $\tilde{\boldsymbol{u}}(\boldsymbol{x})$ online to ensure safety and stability via the CBF and CLF constraints.









